The hot circumgalactic medium in the eROSITA All-Sky Survey III. Star-forming and quiescent galaxies

The circumgalactic medium (CGM), as the gas repository for star formation, might contain the answer to the mysterious galaxy quenching and bimodal galaxy population origin. We measured the X-ray emission of the hot CGM around star-forming and quiescent galaxies. We detect extended X-ray emission from the hot CGM around star-forming galaxies with $\log(M_*/M_\odot)>11.0$ and quiescent galaxies with $\log(M_*/M_\odot)>10.5$, extending out to $R_{\rm 500c}$. $L_{\rm X, CGM}$ of star-forming galaxies with median stellar masses $\log(M_{\rm *,med}/M_\odot) = 10.7, 11.1, 11.3$ are approximately $0.8\,, 2.3\,, 4.0 \times 10^{40}\,\rm erg/s$, while for quiescent galaxies with $\log(M_{\rm *,med}/M_\odot) = 10.8, 11.1, 11.4$, they are $1.1\,, 6.2\,, 30 \times 10^{40}\,\rm erg/s$. Notably, quiescent galaxies with $\log(M_{\rm *,med}/M_\odot) > 11.0$ exhibit brighter hot CGM than their star-forming counterparts. In halo mass bins, we detect similar X-ray emission around star-forming and quiescent galaxies with $\log(M_{\rm 200m}/M_\odot) > 12.5$, suggesting that galaxies in the same mass dark matter halos host equally bright hot CGM. We emphasize the observed $L_{\rm X, CGM} - M_{\rm 500c}$ relations of star-forming and quiescent galaxies are sensitive to the stellar-to-halo mass relation (SHMR). A comparison with cosmological hydrodynamical simulations (EAGLE, TNG100, and SIMBA) reveals varying degrees of agreement, contingent on the simulation and the specific stellar or halo mass ranges considered. Either selected in stellar mass or halo mass, the star-forming galaxies do not host brighter stacked X-ray emission from the hot CGM than their quiescent counterparts at the same mass range. The result provides useful constraints on the extent of feedback's impacts as a mechanism for quenching star formation as implemented in current cosmological simulations.

==> extra-text.tex <==
Considering the conclusion we drew that the halo mass is the dominant parameter to decide the X-ray luminosity of the hot CGM, we compare the SHMR in the three simulations to the SHMR of the stacked galaxies (which is calibrated according to the galaxy lensing survey) \citep{Tinker2021,MandelbaumWangZu_2016MNRAS.457.3200M}.\textcolor{blue}{JC: move this first:} We present the median $M_{\rm 200m}$ and its 16-84\% scatter to the stellar mass relation in the bottom row of Fig.\ref{Fig_sim}. For the quiescent galaxies, the SHMR of the three simulations agrees well with the lensing observation. However, only SIMBA captures the bi-modality feature of the SHMR, namely the star-forming galaxies located in the lower-mass halo. We conclude that the overshooting of the X-ray luminosity of star-forming galaxies in TNG100 and EAGLE is due to the absence of bi-modality in the SHMR \textcolor{blue}{JC: I would say it is a bit too strong?}. Indeed, the joint calibration with the SHMR and $L_{\rm X, CGM}-M_*$ is expected to be implemented in the next-generation simulation suites\textcolor{blue}{JC: previous sentence is unclear to me.}.


%The CGM and feedback processes in galaxy evolution models are currently a strong focus of the community \citep{OppenheimerBabulBahe_2021Univ....7..209O, EckertGaspariGastaldello_2021Univ....7..142E}. 
%the existing gas reservoir within reach of galaxies
%in the range of $10^{10}<$M$^*/$M$_\odot<3\times10^{11}$,  \citep{Truong2020, DaviesCrainOppenheimer_2020MNRAS.491.4462D}. 

%Theoretically, the strong influence of AGN feedback on the normalization and shape of the L$_X$ or Y scaling relation with halo mass was demonstrated \citep{LeBrunMcCarthySchaye_2014MNRAS.441.1270L}. 
%Recent Illustris TNG simulations show a fair agreement for these scaling relations with observations of clusters of galaxies \citep{PopHernquistNagai_2022arXiv220511528P}.

%The X-ray luminosity of lower-mass haloes will further constrain the feedback processes from AGN and stars. In particular, the scaling relation split as a function of star-forming and quiescent galaxies strongly depends on the feedback \citep{OppenheimerBogdanCrain_2020ApJ...893L..24O, Truong2020, Truong2021a}. 


In the paradigm of hierarchical structure formation driven by gravitation, the primordial density field made of dark matter and baryons undergoes collapse to form virialized objects: halos and galaxies \citep{White1978}. 
Galaxies, halos and their environments co-evolve and their properties are correlated \citep{Muldrew2012}. 
For example, \citet{Leauthaud2012a,Leauthaud2012b} and \citet{Coupon2015} observed a tight relation between the stellar mass ($M_*$) of a galaxy and its host dark matter halo mass ($M_{\rm halo}$). Moreover, galaxies follow a well-known main sequence between star formation rate and stellar mass \citep{Whitaker2012,Iyer2018}, and show a correlation between their size and stellar mass \citep{Mowla2019a,Mowla2019b}. 


In fact, the hot ($T>10^6 K$) phase of the CGM is thought to be the dominant component of the CGM baryon budget; it emits X-rays via collisionally ionized gas line and bremsstrahlung. 
This emission is faint, due to the low density of hot CGM.
From a theoretical perspective, on the one hand the CGM heated by feedback processes may introduce a relationship between the X-ray luminosity of the hot CGM ($L_X$) and galaxy properties like \textit{(i)} stellar mass $M_*$, \textit{(ii)} star formation rate (SFR), \textit{(iii)} presence or absence of AGN, \textit{(iv)} azimuth angle \citep[e.g.][]{Truong2020, Truong2021a, Truong2021b}; 
on the other hand, the hot CGM heated by accretion shocks may introduce a relationship between $L_X$ and dark matter halo mass $M_{\rm halo}$ (which is not directly observable) \citep[e.g.][]{PopHernquistNagai_2022arXiv220511528P}. 

Pointed observations using {\it Chandra} or {\it XMM-Newton} revealed the hot gas properties of just a few nearby galaxies ($<50$ Mpc)\citep{Strickland2004,Tullmann2006,Wang2010,Li2013b}. 
With their spatial resolution, {\it Chandra} and {\it XMM-Newton} resolve the stellar sources distributed in the disk of nearby galaxies, but,
Unfortunately, their small field of view (FOV) and sensitivity limit the number of galaxies around which the CGM can be detected. 

For the early-type galaxies (ETGs), the relation between $L_X$ and $M_*$, dynamical mass (baryon plus dark matter), central optical profile of galaxy and temperature of gas ($T_X$) was studied within $<50$ Mpc \citep{Kim2013,Kim2015,Goulding2016,Forbes2017}. 
The relations measured support the necessity of AGN feedback in massive ETGs and demands of stellar feedback in less massive ETGs \citep{Choi2015}. 
For the late-type galaxies (LTGs), the Chandra survey of nearby ($<30$ Mpc) highly inclined disc galaxies found correlations between $L_X$ and SFR, supernova (SN) mechanical energy input rate and $T_X$, which implies a stellar feedback origin of the X-ray emission \citep{Li2013a, Wang2016}. A weaker correlation between $L_X$ and $M_*$ is found in disk galaxies especially star-burst galaxies, compared to ETGs. 

The hot gas surveys of {\it Chandra} and {\it XMM-Newton} focus on the \emph{inner} hot CGM `corona', with scale-heights of just about 1-30 kpc (median of 5 kpc), where feedback processes dominates over gravitation. 
For the \emph{outer} hot CGM, where the gravitational virialized gas dominates, in order to heat up the gas to X-ray emitting temperature over the radiation cooling curve through gravitation, $M_{\rm halo}$ needs to be massive enough (>$10^{12.7} M_\odot$), which corresponds to massive galaxies with $M_*>10^{11}M_\odot$  \citep[M31-like;][]{Keres2009a,Keres2009b,Voort2016,Li2016}. 

For these reasons, although the hot gas in galaxy groups and clusters has been detected and studied well \citep{Pratt2009,Anderson2015,Li2017}, very few detections of the \emph{outer} hot CGM (out to 70 kpc) from massive galaxies have been reported \citep{Dai2012,Bogdan2013,Bogdan2015, Anderson2016,Li2016}. 
Current samples are too small to build statistically robust correlations between $L_X$ and properties of galaxies, so it is hard to constrain the origin of the hot CGM \citep{Li2017}.

To chart the CGM's outer emission beyond the local Universe, we need to resort to stacking techniques to detect its faint emission, which provides a more general avenue to study correlations between $L_X$ and the properties of galaxies. 
By stacking about 250,000 `locally brightest galaxies’ selected from the Sloan Digital Sky Survey (SDSS) using data from ROSAT All-Sky Survey, \citet{Anderson2015} detected hot gas emission around $M_*>10^{10.8}M_\odot$ galaxies. They found the $L_X-M_*$ relation is steeper than expected from self-similarity theory, implying the existence of non-gravitational heating \citep{Anderson2015}. For the same galaxy sample, a general correlation between the galaxy stellar mass and the Comptonization Y-parameter was measured by \citep{PlanckCollaborationAdeAghanim_2013A&A...557A..52P}. 

Measurements of the CGM with the thermal Sunyaev–Zeldovich (SZ) effect have progressed in the last years thanks to observations from the Atacama Cosmology Telescope \citep{AiolaCalabreseMaurin_2020JCAP...12..047A}. 
With an improved spatial resolution, \citep{SchaanFerraroAmodeo_2021PhRvD.103f3513S,PandeyGattiBaxter_2022PhRvD.105l3526P} measured the $Y$-Mass relation at the high mass end. 
More recently, \citet{DasChiangMathur_2023ApJ...951..125D} have extended the relation down to $M_*>5\times 10^{10}M_\odot$ by cross-correlating the WISE and SuperCOSmos photometric redshift galaxy sample \citep{BilickiPeacockJarrett_2016ApJS..225....5B} with ACT and Planck. 
%With a model, they split the emission into that of the 1-halo and the 2-halo term. 
%They consider systematic uncertainties related to galactic dust, though they might still suffer from contamination by unmasked clusters or groups traced by satellites. 

X-ray stacking experiments are dramatically progressing thanks to extended ROentgen survey with an Imaging Telescope Array (eROSITA), on board the Spektrum Roentgen Gamma (SRG) orbital observatory. 
Launched in 2019, it is a sensitive X-ray telescope performing an all-sky survey with a wide-field focusing telescope \citep{Merloni2012,Predehl2021,SunyaevArefievBabyshkin_2021A&A...656A.132S}. 
The sensitivity of eROSITA is maximal in the soft energy band, i.e., below 2.3 keV, which makes it suitable for studying the million-degrees hot CGM emission. 
Recently, with eROSITA and its PV/eFEDS observations covering just 140 square degrees, \citet{Comparat2022} stacked 16,000 central galaxies selected from the GAMA spectrospcoic galaxy survey; 
later, \citet{Chada2022} stacked 1,600 massive galaxies selected from SDSS in the same eFEDS field. 
Both works detected and measured weak X-ray emission from the outer CGM of those galaxies. 
To date, four of the planned eight all-sky surveys (eROSITA all-sky survey, eRASS:4), each lasting about six months, have been completed. This implies that the amount of the X-ray data available for CGM stacking studies is about 40 times larger than what was available for the eFEDS region (100 times more area covered with about 40\% the exposure time). 

%To control the selection effects and possible contamination from nearby galaxies. The galaxy samples are selected with an aim of 95\% completeness to approximate volume-limited samples. 
%Three methods are applied to handle the contamination from nearby galaxies (environment): We define an `isolated' galaxy sample to minimize the contamination, we define a central galaxy sample from the newest group finder and we model the contamination by stacking satellite and central galaxies separately. With well-defined galaxy samples, we split them to different $M_*$ or $M_{\rm halo}$ bins, star-forming or quiescent galaxy samples and stack the X-ray emission using the eRASS:4 observations. We provide the average X-ray surface brightness profiles around galaxies, star-forming galaxies, quiescent galaxies, dark matter halos over $\log(M_*)=9.5-11.5$ or $\log(M_{\rm halo})=11.5-14.0$.
%The most up-to-date relationships between X-ray luminosity within $R_{\rm vir}$ or $R_{500}$ and galaxy or halo properties are measured. 


The galaxy samples are defined in Sec.~\ref{Sec_galaxy}. 
The models (AGN, XRB) and mock galaxy catalogs are described in Sec.~\ref{Sec_model}. 

\section{Method. Star-forming and quiescent galaxy samples} \label{Sec_method}



%\jc{Add quick summary about the three selections isolated and CEN}

%In Sec. \ref{SubSec_sfqu_fullISO} (\ref{SubSec_sfqu_CEN}), we detail how the separation is done for the Full and isolated (central) galaxy samples. More details are given in Appendix~\ref{Apd_sfqu}.

%\subsection{FULL and isolated galaxy samples}\label{SubSec_sfqu_fullISO}

%We split the `FULL$_{\rm phot}$' sample into star-forming (`SF') or quiescent (`QU') sub-samples to study if they have different X-ray properties.
%The five bands photometry is not sufficient to obtain unbiased and accurate estimates of the star formation rate (SFR) of galaxies. Instead, we split galaxies into the red sequence, green valley and blue cloud populations using the color-magnitude diagram. We take the blue cloud population as `SF' and the red sequence population as `QU'.
%We define the separation between blue cloud and green valley galaxy population as $(g-r)= - 0.055 M_r-\alpha_1$ and the separation between green valley and red sequence galaxy population as $(g-r)= - 0.055 M_r-\alpha_2$  \citep{Liao2023}. %$\alpha_1$ and $\alpha_2$ evolve with redshift \textbf{add ref}. 
%We use GAMA, where the SFR of galaxies are accurately estimated, to derive $\alpha_1$ and $\alpha_2$ and their redshift dependence, see details in Appendix~\ref{Apd_sfqu}. 
%We make sure the purity of the `SF' and `QU' populations is about 90\% and completeness is larger than $>80\%$. 
%The $\alpha_1$ and $\alpha_2$ values obtained and corresponding completeness and purity are listed in Table.~\ref{Tab_purity}. 

%We compare our selections with models of the red sequence from clusters of galaxies \citep{GladdersYee_2000AJ....120.2148G}. We use the models calibrated on LS DR10 following \citet{IderChithamComparatFinoguenov_2020MNRAS.499.4768I}. We find that more than 90\% of the selected `QU' galaxies are indeed in the red sequence and that less than 20\% of the selected `SF' galaxies are in the red sequence classification, see Appendix~\ref{Apd_sfqu}.
%We list the number of galaxies in each stellar mass bin split in `SF' or `QU' in Table~\ref{Tab:gal:samples}. 

\section{star-forming and quiescent population definition of LS DR9}
\label{Apd_sfqu}

\begin{figure}
     \centering
         \includegraphics[width=0.8\columnwidth]{fig/apd/DR9_GAMA_color.png}
        \caption{The color-magnitude diagram of the LS DR9 sample matched to GAMA at $z<0.1$. The color of the dots denote the star-forming or quiescent defined in GAMA. The line separate the star-forming (below line) or quiescent (above line) galaxies in LS DR9.}
        \label{Fig_gama_dr9_color}
\end{figure}

\begin{table*}[h]
\begin{center}
\caption{The completeness and purity of star-forming and quiescent population definition}
\label{Tab_purity}
\begin{tabular}{c|ccc|cccc} 
\hline
\hline
&&star-forming&&&quiescent&\\

&$\alpha_1$&purity&completeness&$\alpha_2$&purity&completeness\\
\hline
z<0.1&0.37&90\%&91\%&0.34&88\%&78\%\\
0.1<z<0.2&0.33&89\%&76\%&0.29&89\%&90\%\\
0.2<z<0.3&0.12&88\%&79\%&0.06&88\%&85\%\\
0.3<z<0.4&-0.02&87\%&70\%&-0.08&90\%&92\%\\
\end{tabular}
\tablefoot{The redshift bins, derived $\alpha_1$ ($\alpha_2$), purity and completeness of `SF' (`QU') samples compared to GAMA catalog.}
\end{center}
\end{table*}

\begin{table}[h]
\begin{center}
\caption{The purity of star-forming and quiescent population compared to red sequence model}
\label{Tab_purity_rs}
\begin{tabular}{cccc} 
\hline
\hline
{$\rm log_{10}(M_*/M_\odot)$} & star-forming&quiescent\\
\hline
(9.5,10.0)&97\%&90\%\\
(10.0,10.5)&90\%&98\%\\
(10.5,11.0)&82\%&96\%\\
(11.0,11.25)&89\%&93\%\\
(11.25,11.5)&78\%&97\%\\
(11.5,12.0)&70\%&99\%\\
\end{tabular}
\tablefoot{The stellar mass bins, the purity of our defined `SF' and `QU' sample compared to the red sequence model derived from galaxy cluster.}
\end{center}
\end{table}

We define the `SF' and `QU' samples of LS DR9 catalog according to the color magnitude diagram.
We use GAMA to constrain the separation of `SF' and `QU' samples in the color magnitude diagram. 
With SED fitting, GAMA catalog provides accurate estimation of SFRs of galaxies. We define GAMA galaxy with specific star formation rate $log(sSFR)> -10.5 yr^{-1}$ as star-forming galaxy and $log(sSFR)< -10.5 yr^{-1}$ as quiescent galaxy \citep{Belfiore2018}.
%This definition gives similar SMF to \citet{Kelvin2014}

We take the matched galaxies in Section.~\ref{Apd_dr9_gama_cat}.
The quality of `SF' and `QU' sample definition is quantified by the purity and completeness. 
The purity is defined as the percentage of LS DR9 galaxies identified as `SF' and `QU' also in GAMA. The completeness is defined as the percentage of `SF' and `QU' in GAMA also in LS DR9.

We fix the slope of the separation and change $\alpha_1$ and $\alpha_2$ to find the values where the purity of `SF' and `QU' samples is about 90\% and not losing the completeness.
The magnitude we used have considered Galactic extinction \citep{Zou2019}. The results at different redshift bins are listed in Table.~\ref{Tab_purity}.
As an example, the color-magnitude diagram of matched galaxies at $z<0.1$ is plotted in Fig.~\ref{Fig_gama_dr9_color}.
We then applied another check by comparing to the red sequence model defined in . We take the definition of red sequence and calculate the purity again, the result is listed in Table.~\ref{Tab_purity_rs}.
%GAMA can be split to blue/green/red galaxies according to the colour– mass diagram \citep{Prescott2011}. The separation between blue and green (green and red) is $(g-i)=0.03\times log(M_*) +0.45 (0.4)$. 
%The two definitions agree with each other, as plotted in Fig.`\ref{Fig_gama_rgb}'
In general, our LS red sequence galaxy is well defined with high purity and completeness.

%\section{Needed $z_{spec}$ to selection central galaxy} \label{Apd_specz}

%We define central galaxy as the most massive galaxy that has no intersect within two times of its virial radius in space. We find even using spectroscopic survey that can estimate redshift with $\Delta z<0.0001$, there are still $>30\&$ satellite galaxies wrongly pass the central galaxy selection. Therefore with the LS DR9 galaxy catalog where $\Delta z \approx 0.01$, it is impossible to separate central and satellite galaxies correctly. 

%Besides, we add the typical error of spectropic redshift ($\Delta z_{spec}=0.0001$ \citep{Driver2022,Strauss2002,Thomas2013}) to Uchuu catalog and do the 3D selection, the HOD is plotted in . 


The LS DR9 covers 14,000 deg$^2$ of extragalactic sky. 
The overlap with the X-ray observations detailed above is 9,340 deg$^2$. 
We use the galaxy catalog from \citet{Zou2019,Zou2022}\footnote{In this work, we use 'LS DR9' to refer to the galaxy catalog from \citet{Zou2019,Zou2022}.}. 
This catalog uses three optical bands (g,r,z) from CTIO/DECam and two infrared bands (W1, W2) from WISE photometry. 
They select galaxies with $r_{AB}<23$, S/N>10 and the morphology of the galaxy is not point source like.

\citet{Zou2019} estimate the photometric redshift ($z_{phot}$) using local linear regression algorithm \citep[LePhare,][]{ArnoutsCristianiMoscardini_1999MNRAS.310..540A, IlbertArnoutsMcCracken_2006A&A...457..841I}. 
The bias of $z_{phot}$ defined as the median offset between $z_{phot}$ and spectroscopic redshift $z_{spec}$ is $(z_{phot}-z_{spec})/(1+z_{spec})=-4\times10^{-4}$ and the dispersion is $\Delta z_{phot}=0.01$. 
The stellar mass ($M_*$) of galaxies is calculated by spectra energy distribution (SED) fitting with theoretical stellar population synthesis models from \citet{BruzualCharlot_2003MNRAS.344.1000B} at the photometric redshift. 
The dispersion of $\log_{10}(M_*[M_\odot])$ compared to COSMOS is $\sim$0.2 dex. 
We match LS DR9 galaxies to the GAMA galaxy catalog. We confirm the bias and dispersion values of redshift and stellar mass quoted by \citet{Zou2019}, see Appendix \ref{Apd_dr9_gama_cat}. 

The nearby galaxies with a large extent on the sky need special treatment in the DESI legacy survey as summarised in the Siena Galaxy Atlas (SGA) catalog \citep{MoustakasLangDey_2023arXiv230704888M}. 
We found about 16k nearby galaxies in SGA are missing in the LS DR9 catalog (due to the initial selection explained above). We add them to the catalog, see detail is in Appendix~\ref{Apd_SAG}. 

We measure the galaxy stellar mass function (GSMF) of the LS DR9 catalog and compare it to spectroscopic surveys: COSMOS, GAMA and SDSS. We find good agreement for stellar masses larger than $10^{10}$M$_\odot$, see Appendix.~\ref{Apd_dr9_gama_smf}.

\subsection{Full$_{\rm phot}$ galaxy sample}\label{Sec_full}

On the LS DR9 catalog, for the galaxy with both $z_{\rm spec}$ and $z_{\rm phot}$ measurements, we take $z_{\rm spec}$ and name the new redshift as `Z\_BEST'. 
We apply the selection criterion below:

We split the galaxy sample into five stellar mass bins as listed in Table.~\ref{Tab:gal:samples}. 
We name the $\log(M_*)=10.5-11.0$ bin as `MW-mass' bin, the $\log(M_*)=11.0-11.25$ bin as `M31-mass' bin and the $\log(M_*)=11.25-11.5$ bin as `2M31-mass' bin. 
Constrained by the PSF of eROSITA, we take different maximum redshifts for each mass bin, see Table.~\ref{Tab:gal:samples}. 
Considering that the hot CGM of very local galaxies may extend across a large area over sky and complicate background subtraction, we leave them for specific study in the following work. We take minimum redshift $z_{min}=0.01-0.03$ for galaxy samples at different $M_*$ bins. 
%avoid possible biases due to the in-homogeneity of the local Universe within a 130 Mpc sphere
We obtain 1677909 galaxies that constitute the `FULL$_{\rm phot}$' sample. 

\subsection{Isolated galaxy sample (isolated)}\label{Sec_iso}

We define an `isolated' galaxy sample from the FULL$_{\rm phot}$ sample to minimize the projected X-ray emission from nearby galaxies. 
%For each pair of galaxies, if the angular separation of a galaxy pair is smaller than the sum of their virial radii, namely if there is an overlap of their virial halo, we only keep the galaxy with $M_*$ at least twice larger than any surrounding galaxies. 
Considering the dispersion of the $z_{phot}$ and $M_*$ of LS DR9, we enlarge the `FULL$_{\rm phot}$' galaxy sample by $z_{phot}<z_{max}+0.05$ and $M_*>1/2M_{min}$ to avoid extra selection of isolated galaxy. 

The fraction of isolated galaxies in the FULL$_{\rm phot}$ sample is 25\% at the lower mass end, 17\% for MW-mass bin, 8\% for M31-mass bin and 5\% for mass bin 11.25-11.5.
Table \ref{Tab:gal:samples} details the total number of isolated galaxies obtained for each sample. In total, we have 213514 isolated galaxies. The size of the isolated galaxy sample is about 13 times larger than \citet{Comparat2022}, 130 times larger than \citet{Chada2022} and close to the sample size of \citet{Anderson2015}.


\subsection{Central galaxy sample}\label{Sec_cen}

We consider the galaxy catalog based on SDSS Main Galaxy Sample (MGS), where the self-calibrated halo-based group finding algorithm is applied to classify the galaxy as central or satellite and estimate the halo mass \citep{Tinker2021, Tinker2022}. The algorithm is slef-calibrated using the observation including the 
The group finding algorithm assigns halos to self-calibrated galaxies by comparing the catalog to complementary data \citep{Tinker2021}. The algorithm's performances are very good: The halo masses of either star-forming or quiescent central galaxies agree well with the halo masses estimated from weak-lensing observation. The clustering properties (HOD, $M_{\rm h}-M_*$ relation) of star-forming or quiescent galaxies are well reproduced \citep{Tinker2022}.

MGS is more than 95\% complete down to r band magnitude of 17.77 \citep{Strauss2002, AbazajianAdelman-McCarthyAgueros_2009ApJS..182..543A} and overlaps with eROSITA observations on about 4,010 square degrees.  
The galaxy sample with $\log(M_*)>11.0\ (10.0)$ is complete within $z<0.15$ ($z<0.06$). 
Compared to the FULL$_{\rm phot}$ and isolated samples, it covers a smaller volume due to a limited redshift reach and a smaller area. However, the knowledge of the galaxy catalog is better, i.e., the AGN population.

For each galaxy in the catalog, its classification as central (\texttt{P\_sat} < 0.5) or satellite (\texttt{P\_sat} $\ge$ 0.5) and its host halo mass (\texttt{M\_halo}) is estimated. 
The star-forming (\texttt{color\_flag}=0) or quiescent (\texttt{color\_flag}=1) classification is estimated based on the measurements of the 4000\AA \ break from \citet{BrinchmannCharlotWhite_2004MNRAS.351.1151B} and the stellar masses are taken from \citet{ChenKauffmannTremonti_2012MNRAS.421..314C}.
The SF/QU definition differs from the color-magnitude diagram for the FULL$_{\rm phot}$ and isolated samples. 


\subsection{Central galaxy sample}%\label{Sec_cen}
\label{SubSec_sfqu_CEN}

We consider the galaxy catalog based on SDSS Main Galaxy Sample (MGS), where the self-calibrated halo-based group finding algorithm is applied to classify the galaxy as central or satellite and estimate the halo mass \citep{Tinker2021, Tinker2022}. 
The star-forming (\texttt{color\_flag}=0) or quiescent (\texttt{color\_flag}=1) classification is estimated based on the measurements of the 4000\AA \ break from \citet{BrinchmannCharlotWhite_2004MNRAS.351.1151B} and the stellar masses are taken from \citet{ChenKauffmannTremonti_2012MNRAS.421..314C}.
The SF/QU definition differs from the color-magnitude diagram for the FULL$_{\rm phot}$ and isolated samples. 

\subsubsection*{Galaxy sample in stellar mass bins (CEN)}

The galaxy samples selected from the SDSS MGS in stellar mass bins are listed in Table \ref{Tab:gal:samples}. We name the central (satellite) galaxy sample here as `CEN' (`SAT') sample. We limit $10<\log(M_*)<11.5$, as below and above the galaxy samples are too small. 
The maximum redshift is limited so that the galaxy sample is complete. Due to the bright SDSS selection ($r_{\rm AB}<17.77$), it turns out to be smaller than the $z_{3\times PSF}$. 
In total, we have 85222 central galaxies, about 40\% of the isolated sample size.

There are two main differences between the isolated sample and CEN sample. First, the isolated galaxies are central galaxies with at most $M_{\rm sat}=1/2 M_{\rm cen}$ satellites in the halo and the satellite boost is well removed. Therefore, the isolated galaxies are located in a more sparse environment than the central galaxy sample and should be considered as a subsample of the central galaxy population.
Second, the redshift distributions of the isolated and CEN samples are different. Therefore, when comparing the stacking results of the two samples, the redshift evolution needs to be considered, especially for the point sources AGN and XRB.

%The algorithm may remain imprecise in assigning the halo center at the high mass end (log$(M_*)>11.5$, log$(M_{200})>14$), which therefore we do not study here. 

%The redshifts are more accurate than measurement in sample is different with the isolated sample, which can be used for a double check of the stacking.

\subsubsection*{Galaxy sample in halo mass bins (CEN$_{\rm halo}$)}\label{Sec_dmhalo}

The hot CGM is heated by the feedback processes from the galaxy (related to $M_*$ and SFR) and the accretion shock within the halo (related to $M_{\rm halo}$). The two mechanisms complicate the interpretation of the stacking result in $M_*$ bins.
For example, the star-forming or quiescent galaxies with the same $M_*$ reside in dark matter halos with different $M_{\rm halo}$, meaning both feedback and shock heating are different, which one takes the role is hard to constrain.

With halo mass assigned to each galaxy in the SDSS MGS by the group finder algorithm, we can study how the $M_{\rm halo}$ is related to the X-ray emission of galaxies.
We define a halo mass selected sample (we name it as CEN$_{\rm halo}$ sample.), by splitting it into five bins ranging in $M_{halo}=11.5-14.0$ every 0.5 dex, see Table.~\ref{Tab:gal:samples}. 
%We calculate the median stellar mass of galaxies in each halo bin, 
The maximum redshift for each sample is set where these galaxy sample's completeness is at 90\% complete (for magnitude cut $r_{AB}=17.77$). 
%Notice the $M_*$ distribution of the central galaxies in each dark matter halo bin is scattered, ranging from $log(M_*)=8.5-12.0$.
The bins containing less than 1000 galaxies will not be stacked. In total, we have 125512 central galaxies in the CEN$_{\rm halo}$ sample.

\section{Models}\label{Sec_model}


%More detail of the reliability examination of the light cone is in \citet{Dong2022}.
%\subsubsection{Testing isolated selection}
We build a mock LS DR9 catalog from the light cone to z=0.45. We apply the magnitude cut $r_{AB}<21$ to the light cone. We add a Gaussian distributed $z_{\rm error}$ and $M_{\rm error}$ with the same median and dispersion of LS DR9 catalog to the accurate ones from the mock catalog. 
We derive the $R_{vir}$ of galaxies using the same method in Sect.~\ref{Sec_iso}.
As a first verification, we calculate the galaxy stellar mass function (GSMF) of this mock LS DR9 catalog and compare it to LS DR9. They agree well, the detail is in Appendix~\ref{Apd_dr9_gama_smf}. 

We use the mock LS DR9 catalog to assess the isolated selection effect of our galaxy samples, as mentioned in Sect.~\ref{Sec_iso}.
We also use the mock LS DR9 catalog to derive the average underlying $M_{\rm halo}$ and $R_{\rm vir}$ of stacked galaxies. Specifically, the average $R_{\rm vir}$ of the quiescent galaxy is larger than the star-forming galaxy with the same $M_*$. We use that value of $R_{\rm vir}$ to define the integration boundary of the X-ray surface brightness to calculate $L_{\rm X}$. 

Similarly, we build a mock SDSS MGS catalog. We apply the magnitude cut $r_{AB}<17.77$ and add a Gaussian distributed $z_{\rm error}=10^{-4}$ and $M_{\rm error}=0.01\ \rm dex$ to the accurate ones from the mock catalog. 

\subsection{Models for AGN and XRB emission}\label{Sec_agnxrb}

Both AGN and XRB emit X-ray. The PSF and sensitivity of eROSITA prevent us to resolve all point sources at the redshift we stack. 
Therefore, to infer what fraction of the measured X-ray emission comes from the hot CGM, we need to build reliable AGN and XRB models and predict their emission. 
We opt for an empirical model to predict the XRB X-ray emission based on the stellar mass and SFR of galaxies (Sec.~\ref{Sec_xrb}). 
For the AGN, we opt for an observation-based approach. We stack galaxies identified as hosting AGN by the BPT diagram and estimate the AGN emission (Sec.~\ref{Sec_agn}).


\subsubsection{Model for XRB}\label{Sec_xrb}

The X-ray luminosity of XRB in the 2-10 keV band ($L_{\rm 2-10keV}$) scales with the star formation rate and stellar mass of host galaxies \citep{Lehmer2016,Aird2017}. 
We predict the $L_{\rm 2-10keV}$ and estimate its uncertainty using models in \citet{Aird2017}. We convert $L_{\rm 2-10keV}$ to the X-ray luminosity in 0.5-2 keV ($L_{\rm XRB}$) by assuming an absorbed (with nH column density at $4\times10^{20}\rm cm^{-2}$, the median nH of the stacked area) power law with a photon index of 1.8. The average SFR of the isolated galaxy sample is estimated using the mock LS DR9 catalog. We take the SFR of galaxies in SDSS MGS estimated by \citet{Brinchmann2004} to predict the XRB emission of the `CEN' sample. 

\subsubsection{Model for AGN}\label{Sec_agn}

We consider galaxies identified as `AGN' or `composite' using the BPT diagram applied to the SDSS MGS central galaxies and name these galaxies as 'CENAGN' sample \citep{BPT1981,Brichmann2004}. 
Depending on the stellar mass, $f_{\rm AGN}=$8-18\% of the CEN are selected as CENAGN, see Table.~\ref{Tab_cenagn}. 
We stack the `CENAGN' sample, and we mask all detected X-ray sources to calculate the maximum X-ray emission from unresolved AGN and XRB as described in Appendix.~\ref{Apd_agn}. We estimate the maximal AGN emission ($L_{\rm AGN,max}$) as the residual emission after subtracting the XRB emission. Under the assumption of no other galaxies hosting AGN, the lower limit of the average AGN contamination in the `CEN' sample is $L_{\rm AGN,max}\times f_{\rm AGN}$. To be conservative, we take the upper limit of AGN contamination as $2\times L_{\rm AGN,max}\times f_{\rm AGN}$; this accounts for (obscured) X-ray AGN not being identifed as AGN or composite in the SDSS spectra. We repeat the procedure for the `CEN$_{\rm halo}$' sample to estimate the AGN contamination there.
%We can only overestimate the AGN, as the BPT diagram selects the star-forming galaxies, where the AGN incidence is about 10 times higher than quiescent galaxies \citep{Aird2018}. 
We find after applying the masks, the unresolved AGN contamination is about 25-50\% of XRB emission. 

As we discussed, the AGN and XRBs located in the satellites would contaminate the hot CGM emission attributed to the central galaxy. 

We take the mock LS DR9 and SDSS MGS catalog to evaluate the satellite galaxy distribution. 
For each stacked galaxy, we select the galaxy with similar stellar mass (difference smaller than 0.1 dex) and redshift (difference smaller than 0.01) in the mock catalog. We count the number of satellite galaxies and the projected distances of the satellites to the mock central galaxy. 
The XRB emission of the satellite is estimated based on its $M_*$ and SFR. The AGN population in satellite galaxies is unclear, there could be 0-20\% satellite galaxies hosting AGN \citep{Comparat2023}. Here we assume the AGN contamination in the satellite galaxies is negligible after applying masks.
We sum and average the XRB emission in satellites as a function of distance to the central galaxy. 
The X-ray luminosity of XRB in the satellites is estimated by summing up the satellites in the same radius of stacking, i.e. $R_{500}$. 

The model of unresolved point sources in satellites is necessary, especially for massive galaxies. We find the total X-ray luminosity of unresolved XRBs in satellites is about 8\% (19,37,66\%) of the XRB in the central galaxy, for the four $M_*$ bins in CEN sample. 

The satellite galaxy might be misclassified as a central galaxy in the group finder with a chance of <1\% \citep{Tinker2021}. 
%In the case of halo mass selection (CEN$_{\rm halo}$), the effect of it is negligible. 
In the case of stellar mass selection (CEN), since satellites are hosted by more massive (brighter in X-ray) haloes, the contamination can not be ignored.
Here we consider the 1\% satellite galaxies in the CEN sample and model their contamination. We stack galaxies and measure the X-ray emission in the SAT sample ($S_{\rm X,SAT}$). We rescale the X-ray profiles of CEN ($(S_{\rm X,CEN}$) as $(S_{\rm X,CEN}-1\% S_{\rm X,SAT})/99\%$. The rescaled X-ray luminosity of CEN drops by about 5\%.
%make up 0.5 and 1\% of the number of galaxies in stacks and give an upper limit of the possible contamination due to misclassified centrals as satellites. 



\section{Result. X-ray surface brightness profile}%

\jc{here do a subsection for each selection full first, then isolated and central}
\subsection{Around galaxies from the FULL$_{\rm phot}$ sample}
\label{Sec_profile_full}


\jc{here do a subsection for each selection full first, then isolated and central}
\subsection{Around galaxies from the FULL$_{\rm phot}$ sample}
\label{subSec_profile_full}

\begin{figure}[h]
    \centering
    \includegraphics[width=1.0\columnwidth]{fig/profile/profile_nomask_full_MW_galsfqu.png}
    \caption{Top: The X-ray surface brightness profiles of the FULL$_{\rm phot}$ sample after subtracting background, without masking sources for galaxies with $\log(M_*)=10.0-10.5$, 10.5-11.0 (MW-mass) and 11.0-11.025 (M31-mass). The dotted line is the PSF of eROSITA, 
    vertical dash line denotes the average virial radius of stacked galaxies. The X-ray emission comprises all effects mentioned in Sec.~\ref{Sec_proj}, which limits its interpretability in terms of CGM emission.
    Bottom: The average X-ray surface brightness profiles of MW-mass galaxies, MW-mass star-forming (SF, blue) galaxies, and quiescent (QU, red) galaxies. }
        \label{Fig_profile_full_nomask}
\end{figure}

We take the galaxies in the MW-mass bin as an example, see FIg. \ref{Fig_profile_full_nomask}. 
The X-ray surface brightness profile of the SF sample, which contains fewer satellite galaxies (<20\%), is less extended than the profiles of the QU sample, whose emission is boosted due to the 42\% satellite galaxies located in more massive dark matter halo. We will further discuss that the difference between SF and QU shown here is not an intrinsic property but induced by the satellite boost: if stacking only the central SF or QU sample, we do not detect the difference caused by satellite boost anymore (see Sec.~\ref{Sec_sfqu}). 
Within 10 kpc, star-forming galaxies are on average brighter than quiescent galaxies by almost a factor of 2. This is due to a higher incidence of AGN and XRB in star-forming galaxies. 
%Beyond 10 kpc, quiescent galaxies are brighter and host more extended X-ray halo, compared to star-forming galaxies. 
As only 25\% galaxies in MW-mass bin are star-forming galaxies, the average X-ray surface brightness of galaxies in MW-mass bin is closer to that of quiescent galaxies. 


\subsection{Around galaxies from the isolated and central sample}
\label{subSec_profile_isoCen}

We now focus on the isolated and CEN samples where the satellite boost that hampers the interpretation of the full stacks is minimized.


%\section{Is the X-ray emission around star-forming and quiescent galaxies different?}
%\label{Sec_profileDiscussion}
%How the bi-modality of the galaxy population: star-forming and quiescent galaxies, formed is still a puzzle. 
%In this section, we stack the star-forming and quiescent galaxies respectively, to figure out if the X-ray emission around the galaxy has a difference that can shed light on the observed galaxy bi-modality. 

\subsection{Around galaxies from the isolated and central sample}
\label{Sec_profile_isoCen}

\begin{figure}[h]
    \centering
    \includegraphics[width=1.0\columnwidth]{fig/profile/profile_nomask_full_MW_galsfqu.png}
    \caption{Top: The X-ray surface brightness profiles of the FULL$_{\rm phot}$ sample after subtracting background, without masking sources for galaxies with $\log(M_*)=10.0-10.5$, 10.5-11.0 (MW-mass) and 11.0-11.025 (M31-mass). The dotted line is the PSF of eROSITA, 
    vertical dash line denotes the average virial radius of stacked galaxies. The X-ray emission comprises all effects mentioned in Sec.~\ref{Sec_proj}, which limits its interpretability in terms of CGM emission.
    Bottom: The average X-ray surface brightness profiles of MW-mass galaxies, MW-mass star-forming (SF, blue) galaxies, and quiescent (QU, red) galaxies. }
        \label{Fig_profile_full_nomask}
\end{figure}

%Stacking the FULL$_{\rm phot}$ sample without masking any detected X-ray sources introduces the least uncertainty and bias (from X-ray data reduction or galaxy sample compiling) to the results, the measurement is reproducible. 
%The X-ray surface brightness profiles obtained have a high signal-to-noise ratio (S/N). 
%For the MW-mass galaxies, the integrated luminosity measured within each 100 kpcs has a S/N above 100. 
%These high significance measurements benefit from the large number of sources considered, and the large area covered by X-ray observations. 
%The surface brightness profiles of the FULL$_{\rm phot}$ samples in $\log(M_*)=10.0-10.5$, MW-mass and M31-mass (after subtracting the background) are shown in Fig.~\ref{Fig_profile_full_nomask}. 

%The background is $S_{X,bg,1}$. 
%is detected down to about 1\% of background with the significance of ?, thanks to the great statistics due to the large galaxy sample and sky area we stacked. 
%Due to the satellite boost we described in Sect.~\ref{Sec_proj}, the satellite galaxies located in more massive dark matter halo strongly influence the profiles shown in Fig.~\ref{Fig_profile_full_nomask}, resulting in the stacked X-ray emission extending to about 1-2 Mpc (about 5-10 times of $R_{\rm vir}$ of galaxies).
%The X-ray sources contributing in these stacks include AGN, XRB and hot gas emission (intra-cluster medium (ICM), intra-group medium (IGrM), CGM from central and satellite galaxies in different massive halos. 
%The interpretation of these measurements remains complex and hopefully future simulation and modelling effort will enable unambiguous interpretation of all the signal present in these measurements. 
%The X-ray emission come not only from the sources physically connected to the stacked galaxy but also from sources in the satellite galaxies, nearby large scale structures. 

%The galaxies with stellar mass ranges over one magnitude have comparable X-ray emissivity at about 1 Mpc, implies the emission is from similar large scale environment galaxies reside in, instead of the stacked galaxies.

%The measured profiles after splitting into SF and QU are significantly different from the average emission, as shown in the right panel of Fig.~\ref{Fig_profile_full_nomask}.
%The influence of the satellite boost on the X-ray surface brightness profile is further elucidated by separating stacking analyses of star-forming and quiescent galaxies, as shown in the bottom panel of Fig.~\ref{Fig_profile_full_nomask}. 


%We leave for future studies the elaboration of a satellite boost model that will enable the complete extraction of the information in these stacks with high signal-to-noise. The stacking results of the FULL$_{\rm phot}$ are available at CDS and described in the Appendix~\ref{Apd_profiles} \textbf{add link here}.

We now focus on the isolated and CEN samples where the satellite boost that hampers the interpretation of the full stacks is minimized.

%\section{The circum-galactic medium of star-forming and quiescent isolated and central galaxies selected in stellar mass} \label{Sec_profilegal}

%In this section, we mask all identified X-ray point sources, so that the emission from the hot gas component becomes more discernible.
%The observed surface brightness profiles of the isolated and CEN samples are presented in Sec. \ref{Sec_profileisocen}.
%The X-ray emission from the hot CGM emission is modeled and presented in Sec.~\ref{Sec_profileCGM}.


\section{Is the X-ray emission around star-forming and quiescent galaxies different?}
\label{Sec_profileDiscussion}
%How the bi-modality of the galaxy population: star-forming and quiescent galaxies, formed is still a puzzle. 
In this section, we stack the star-forming and quiescent galaxies respectively, to figure out if the X-ray emission around the galaxy has a difference that can shed light on the observed galaxy bi-modality. 

\begin{figure*}
    \centering
    \includegraphics[width=0.33\linewidth]{fig/profile/profile_mask_cen_MW_galsfqu.png}
    \includegraphics[width=0.33\linewidth]{fig/profile/profile_mask_cen_M31_galsfqu.png} 
    \includegraphics[width=0.33\linewidth]{fig/profile/profile_mask_cen_2M31_galsfqu.png}\\
    
    \includegraphics[width=0.33\linewidth]{fig/profile/profile_MW_SFQU_agnxrb_cgm_singlebeta.png}
    \includegraphics[width=0.33\linewidth]{fig/profile/profile_M31_SFQU_agnxrb_cgm_singlebeta.png}
    \includegraphics[width=0.33\linewidth]{fig/profile/profile_2M31_SFQU_agnxrb_cgm_singlebeta.png}
    \caption{Top: The X-ray surface brightness profiles of star-forming (SF, blue) and quiescent (QU, red) central galaxies, after masking X-ray sources. 
    Bottom: The modeled X-ray surface brightness profiles of hot CGM of star-forming and quiescent central galaxies. From left to right: MW-mass, M31-mass and 2M31-mass galaxies.}
        \label{Fig_profile_sfqu}
\end{figure*}

The X-ray surface brightness profiles of MW-mass, M31-mass and 2M31-mass star-forming and quiescent central galaxies are presented in Fig.~\ref{Fig_profile_sfqu} (The profiles of the isolated sample are presented in Apd.~\ref{Apd_profiles}). 
The top row shows the observed X-ray surface brightness after masking X-ray sources and the bottom row shows the modeled CGM surface brightness profiles. 
From the total surface brightness profiles, extended X-ray emission is detected around star-forming and quiescent galaxies. 
For MW-mass, the star-forming galaxies have brighter X-ray emission than quiescent galaxies within 30 kpc, no significant difference is detected in M31-mass galaxies, while quiescent galaxies are brighter than star-forming galaxies in 2M31-mass galaxies.
The slightly brighter X-ray emission in star-forming galaxies is mainly due to the unresolved point sources, which we model and subtract to estimate the X-ray emission of hot CGM. 
After modeling (Fig.\ref{Fig_profile_sfqu} bottom panels), we find hot CGM X-ray emission of star-forming and quiescent galaxies are similar at MW-mass. For more massive galaxies, the CGM surface brightness profile of quiescent galaxies is brighter than that of star-forming galaxies. For the isolated sample, the AGN contamination is uncertain and prevents estimating the hot CGM X-ray emission. 

%The X-ray emission originates from unresolved point sources and hot gas. The origin of brighter emission in star-forming galaxies is possibly multiple: more XRB and higher AGN incidence in the galaxy \citep{Aird2017,Aird2018}, more hot gas heated by the feedback processes \citep{Truong2021a}. The brighter X-ray emission in star-forming galaxies within 30 kpc might imply the first reason, then we can not exclude the contribution from the second one. On the other hand, the quiescent galaxies would be located in the more massive dark matter halo, compared to the same massive star-forming galaxies, which means the X-ray emission from gas heated by accretion shock should be brighter, or the unresolved sources in the satellites are brighter (which might be the reasons of the brighter X-ray emission beyond 100 kpc in M31-mass central galaxies). \gab{Quantify the detection, if can not demonstrate the different factors, then say that this is unknown and that what you mention could be potential sources of the difference, but at the moment it is unclear to which extent each one of them is playing a role. }

%\jc{It could be due to more efficient cooling in the cores of halos hosting SF galaxies.}
%\jc{does this imply that gravity dominates and that for a similar halo mass, the shock heating induces the same temperature of the hot gas regardless of SF/QU ?}


%As the hot CGM is also modulated by host dark matter halo, we plot the numbers of galaxies (split to central or satellite) with $M_{halo}$ of their host dark matter halo. Because we mask out detected galaxy clusters during stacking, here we go up to $M_{halo}=10^{14}M_\odot$, which is about the detection limit of eRASS:4.
%For the stellar mass bin with 0.5 dex, the corresponding $M_{halo}$ is more dispersed, with 1-2 dex difference. The $M_{halo}$ of central galaxies is less dispersed than satellite galaxies, which proves the importance of isolated galaxy selection. There are satellite galaxies locating at more massive dark matter halo left in the sample, its contamination to the stacking result of galaxies above $10^{11}M_\odot$ is negligible, as the satellite and central galaxies live in similar dark matter halo. The contamination to galaxies below $10^{11}M_\odot$ is mostly at outskirt, as the suspicious X-ray emission detected around 1 Mpc. More detail will be discussed in \textbf{discuss satellite contribution.} 


%\subsection{$L_X-M_*$ relations}\label{Sec_lxmsfqu}

\begin{figure*}
    \centering
    \includegraphics[width=1.0\columnwidth]{fig/lxm/lx_m_mask_2d_sfqu_R500.png}
    \includegraphics[width=1.0\columnwidth]{fig/lxm/lx_m_mask_cen_sfqu_R500.png}
    \caption{The X-ray luminosity within $R_{\rm 500}$ after masking X-ray sources ($L_{\rm X,500}$) as a function of $M_*$ for star-forming and quiescent isolated (left) and central (right) galaxies.}
        \label{Fig_lxm_sfqu}
\end{figure*}

\begin{figure}
    \centering
    \includegraphics[width=1.0\columnwidth]{fig/lxm/lx_CEN_agnxrb_cgm_sfqu_singleline.png}
    \caption{The hot CGM X-ray luminosity within $R_{500}$ of central star-forming galaxies (blue) and quiescent galaxies (red), the modeled unresolved AGN and XRB luminosity of star-forming (light green) and quiescent (light orange) as a function of the $M_*$.}
        \label{Fig_lxm_sfqu_cgm}
\end{figure}

The $L_{\rm X,500}-M_*$ (after masking X-ray sources) relations of star-forming and quiescent galaxies for the CEN and isolated samples are presented in Fig.~\ref{Fig_lxm_sfqu}. 
The star-forming galaxy has a smaller halo mass than the quiescent galaxy with the same stellar mass, as a result, the $R_{500}$ of star-forming and quiescent galaxies are different. To keep consistency, we take the $R_{500}$ of quiescent galaxies to calculate $L_{\rm X,500}$.
We find less than $1\sigma$ difference in $L_{\rm X,500}$ between star-forming and quiescent galaxies. 
Only at the higher masses ($\log(M_*)>11,25$), for the CEN sample, we find a discrepancy that quiescent galaxies are two times brighter than star-forming galaxies. 

The $L_{\rm X,CGM}-M_*$ relation and the modeled X-ray luminosity of AGN and XRB of central star-forming and quiescent galaxies are presented in Fig.~\ref{Fig_lxm_sfqu_cgm}. For MW-mass and less massive galaxies, the X-ray luminosity of hot CGM around star-forming and quiescent galaxies has a difference of less than $1\sigma$, for M31-mass and more massive galaxies, quiescent galaxies host brighter hot CGM emission.

The comparison of the $L_{\rm X}-M_*$ relations in star-forming and quiescent galaxies has been studied with eROSITA observation \citep{Comparat2022, Chada2022} and different conclusions were reached. 
Both studies suffer from the satellite boost problem and large uncertainties due to the limited sample size. 
We compare our results to theirs in Appendix~\ref{Apd_comparesfqu} and find the previous studies (albeit with low constraining power) broadly consistent with the results shown here. 
By defining a large galaxy sample, minimizing the satellite boost and carefully modeling unresolved point sources, we provide a more accurate view on $L_{\rm X}-M_*$ for star-forming and quiescent galaxies. 

A complete model of the differences measured in the surface brightness profiles and $L_{\rm X}-M_*$ relations for star-forming and quiescent galaxies requires delicate treatment of the AGN models, XRB models, and satellite galaxy distribution as a function of specific star formation rate, and correspondingly heated gas through feedback, accretion shocks, as well as non-thermal pressure support. Such models are beyond this observational work and are left for future studies. 

%\yi{Add discussion of simulation}

%There are stronger feedback processes in the star-forming galaxies, while the quiescent galaxies are located in more massive dark matter halo. Measurement of the X-ray luminosity of star-forming or quiescent galaxies respectively is helpful in estimating and quantifying the energy budget of different mechanisms and therefore constrain the galaxy evolution models. 


%Generally, at most $M_*$ bins, the two samples give similar results for star-forming and quiescent galaxies. The higher $L_{X,0.5-2 keV}$ in the isolated sample comparing to `CEN' sample might due to the different AGN emission. First, there is redshift evolution of AGN luminosity, that is brighter at higher redshift. Second, the `CEN' sample removes optical quasars, which decreases the AGN emission.
%This is proved by the relationships when all detected sources are masked (see Fig.~\ref{Fig_lxm_sfqu_mask}). When the bright AGNs are masked, the two galaxy samples give more consistent results. 

%Below about $2\times10^{11}M_\odot$, the X-ray luminosity of blue cloud galxy can be explained by XRB and AGN, while above $2\times10^{11}M_\odot$ other sources like hot gas is needed. Above $8\times10^{10}M_\odot$, XRB and AGN in red sequence galaxies are not sufficient to explain the X-ray luminosity, which implies the detection of hot gas halo of MW-mass red sequence galaxies.

%As mentioned in Section.~\ref{uchuu_iso}, $1\%$ star-forming galaxies and $3\%$ quiescent galaxies in the 'Isolated' sample are satellite galaxies. These satellite galaxies may locate in more massive dark matter halo comparing to the galaxies with same $M_*$ but being central. Because the X-ray emission increases with $M_{halo}$, the satellite galaxies have brighter X-ray emission and may bias the $L_X-M_*$ relation. For the bin $log M_* > 11.0$, the central and satellite galaxies are hosted by same dark matter halo (see right panels of Fig.~\ref{Fig_profile_2d}), which means the X-ray surface brightness profile or $L_x-M_* (M_{halo})$ relation of galaxies $log M_* > 11.0$ have no bias. We therefore derive the new $L_X$ of satellite galaxies from the $M_{halo}$ of its host dark matter halo using the $L_x-M_* (M_{halo})$ relation above $M_{halo}=10^{12}M_\odot$. In this calculation, we assumed the satellite galaxies are as bright as in the central of dark matter halo (i.e. central galaxy), which is not true. Therefore the derived $L_X$ of satellite galaxy should be an up-limit.The satellite contribution to $L_x-M_* (M_{halo})$ relation is then calculated by $(L_{sat}-L_X)\times N_{sat}/(N_{gal}-N_{sat})$, where $L_{sat}$ is the average new $L_X$ of satellite galaxies, $N_{sat}$ is the number of satellite galaxies in each $M_*$ bin.The satellite contribution is plotted in the right panel of Fig.~\ref{Fig_Lx_M}. For the star-forming galaxies, the satellite contribution is only $10\%$, which can be ignored. For the quiescent galaxies, above $log(M_*)=10.6$, the satellite contribution can be ignored, while below $log(M_*)=10.6$, the satellite contribution up-limit is close to the stacked $L_X$. Detailed modelling of satellite contribution will be in following work.

%As only about $30\%$ galaxies are kept in the 'Isolated' galaxy sample, it means the stacking result can not represent the general hot gas properties of galaxy population. On the other hand, the 'Isolated' sample we defined minimises the contamination from projected nearby galaxies and intergalactic medium. The stacked hot X-ray emission relates to the property of the 'Isolated' galaxy and resided dark matter halo only, without interplaying like striping with other galaxies. The result can be compared to the previous XMM-Newton or Chandra observation of CGM of nearby bright galaxies directly.

%From Fig.~\ref{Fig_profile_2d}, the empirical PSF drops to about 10\% within 50 kpc. In the bottom panel of Fig.~\ref{Fig_Lx_M}, we plot the X-ray luminosity in 50-300kpc as a function of stellar mass, that the emission from XRB, AGN is excluded and only extended hot gas emission beyond 50 kpc is plotted. Below $10^{11}M_\odot$, the X-ray luminosities of both blue cloud and red sequence galaxies drop about one magnitude, showing low signal of hot gas emission beyond 50 kpc. Above $10^{11}M_\odot$, the hot gas emission is prominent, with higher emission around red sequence galaxies. 

%\subsection{\jc{LX - stellar mass relation}}This section goes beyond Anderson et al. 2015. full relation integrated in rVir, with all samples spec Z and photoZ. Quantify detection of CGM after subtracting AGN and XRB components

%\subsection{\jc{SF and QU galaxies}} This section goes beyond Comparat et al. 2022. Show profiles and scaling relations


%\subsection{\jc{Focus on MW-like haloes}}Compare profiles


%Note that the contribution from generally uniformly distributed background and foreground galaxies is already removed as background. The projection effect here comes from the local galaxy pairs or groups, namely the local environment of the galaxy.

%If we have more accurate spectroscopic redshift of galaxy, we can precisely build the central galaxy catalog. But considering the error of the photometric redshift of DR9 is about 0.01, namely 40 Mpc, the defined central galaxies are not accurate, there might be some satellite galaxies not removed or wrongly removed. 

%This experiment illustrates the different environment of blue and red galaxies, that redder galaxies tend to locate in denser environments, while reverse for bluer galaxies, consistent with the measurements of the galaxy two-point correlation function and halo occupation distribution function (HOD).


\section{SF/QU in halo mass bins}
\label{Sec_sfQUMhalo}
\begin{figure*}
    \centering
    \includegraphics[width=1.0\columnwidth]{fig/profile/profile_mask_cen_MW_galsfqu_halo.png}
    \includegraphics[width=1.0\columnwidth]{fig/profile/profile_mask_cen_M31_galsfqu_halo.png}
    \caption{\jc{use the MW-mass, M31-mass formalism to be clearer}}
        \label{Fig_profile_halo_sfqu}
\end{figure*}

\begin{figure}
    \centering
    \includegraphics[width=1.0\columnwidth]{fig/lxm/lx_m_halo_mask_cen_sfqu_R500.png}
    \caption{Left: The X-ray luminosity within $R_{500}$ as a function of the $M_{\rm halo}$ for dark matter halos ting star-forming or quiescent central galaxies respectively. The dashed line is a linear relation for illustration and does not fit the data. }
        \label{Fig_lxm_halosfqu}
\end{figure}


By binning the galaxies with the halo mass, the gas heated by accretion would be the same for star-forming and quiescent galaxies, assuming the halo mass determines the properties of accretion shock (though on the other hand, the stellar mass of would be different).
The X-ray surface brightness profiles of star-forming and quiescent galaxies located in dark matter halo with $M_{\rm halo}=12.0-12.5\ (12.5-13.0)$ are compared in Fig.~\ref{Fig_profile_halo_sfqu}. 
The star-forming galaxies are brighter than the quiescent galaxies. The reason might be different for the two halo mass bins. For the $M_{\rm halo}=12.0-12.5$ bin, the unresolved point sources in the stacked star-forming galaxies contribute to the brighter emission, as we do not detect differences beyond 100 kpc. For the $M_{\rm halo}=12.5-13.0$ bin, though the difference is within 1$\sigma$, the profile of the star-forming galaxy is brighter and flatter than the quiescent galaxy, which might imply the stronger feedback heating process, either AGN or stellar, in the star-forming galaxies (or more unresolved point sources in the satellites). \gab{Can you demonstrate it?}


The $L_{\rm X}-M_{\rm halo}$ relations for star-forming and quiescent galaxies are compared in Fig.~\ref{Fig_lxm_halosfqu}. The star-forming galaxy is brighter than the quiescent galaxy, with a maximum difference of 2$\sigma$. Notice the X-ray luminosity includes emission from unresolved AGN and XRB sources and hot gas.
%The reason is due to brighter AGN or XRB, or higher hot gas emission heated by stronger feedback. 
The $L_{\rm X}-M_{\rm halo}$ relations for star-forming and quiescent galaxies are quasi-linear (). \yi{add fit here} 


\section{Summary and conclusions}
\label{Sec_summary}
We use the eRASS:4 X-ray data in the sky area of about 11,000 square degrees, the galaxy samples built from LS DR9 and SDSS galaxy catalogs containing about 213514 isolated galaxies and 85222 central galaxies split into stellar mass bins, 125512 central galaxies split in halo mass bins.
No significant difference between the X-ray emission (from hot CGM and unresolved sources) around the star-forming and quiescent galaxies is detected. After modeling the unresolved point sources, the quiescent galaxies host bright hot CGM emission for M31-mass and more massive galaxies.



The eROSITA sky survey yields a vast repository of X-ray data across the sky, with abundant information on the hot CGM that invites further investigation and analysis. The measured X-ray surface brightness profiles of the FULL$_{\rm phot}$ have a high signal-to-noise ratio, which allows for building a complete model including the galaxy distribution and X-ray properties of the galaxy (Shreeram et al. in preparation).
By knowing the position angle of galaxies, we can study the azimuthal angle dependence of the hot CGM (Zhang et al. in preparation). 
With deeper galaxy surveys, i.e. 4MOST, we can enlarge the galaxy sample, increase the statistics, and obtain a better view of the hot CGM around dwarf galaxies ($\log(M_*)<10$). 



\begin{acknowledgements}

This work is based on data from eROSITA, the soft X-ray instrument aboard SRG, a joint Russian-German science mission supported by the Russian Space Agency (Roskosmos), in the interests of the Russian Academy of Sciences represented by its Space Research Institute (IKI), and the Deutsches Zentrum für Luft- und Raumfahrt (DLR). The SRG spacecraft was built by Lavochkin Association (NPOL) and its subcontractors, and is operated by NPOL with support from the Max Planck Institute for Extraterrestrial Physics (MPE).\\

The development and construction of the eROSITA X-ray instrument was led by MPE, with contributions from the Dr. Karl Remeis Observatory Bamberg \& ECAP (FAU Erlangen-Nuernberg), the University of Hamburg Observatory, the Leibniz Institute for Astrophysics Potsdam (AIP), and the Institute for Astronomy and Astrophysics of the University of Tübingen, with the support of DLR and the Max Planck Society. The Argelander Institute for Astronomy of the University of Bonn and the Ludwig Maximilians Universität Munich also participated in the science preparation for eROSITA.\\

The eROSITA data shown here were processed using the eSASS/NRTA software system developed by the German eROSITA consortium. \\


\end{acknowledgements}

\bibliographystyle{aa}
\bibliography{ref.bib}

\begin{appendix} %First appendix

\section{star-forming and quiescent population definition of LS DR9}
\label{Apd_sfqu}

\begin{figure}
     \centering
         \includegraphics[width=0.8\columnwidth]{fig/apd/DR9_GAMA_color.png}
        \caption{The color-magnitude diagram of the LS DR9 sample matched to GAMA at $z<0.1$. The color of the dots denote the star-forming or quiescent defined in GAMA. The line separate the star-forming (below line) or quiescent (above line) galaxies in LS DR9.}
        \label{Fig_gama_dr9_color}
\end{figure}

\begin{table*}[h]
\begin{center}
\caption{The completeness and purity of star-forming and quiescent population definition}
\label{Tab_purity}
\begin{tabular}{c|ccc|cccc} 
\hline
\hline
&&star-forming&&&quiescent&\\

&$\alpha_1$&purity&completeness&$\alpha_2$&purity&completeness\\
\hline
z<0.1&0.37&90\%&91\%&0.34&88\%&78\%\\
0.1<z<0.2&0.33&89\%&76\%&0.29&89\%&90\%\\
0.2<z<0.3&0.12&88\%&79\%&0.06&88\%&85\%\\
0.3<z<0.4&-0.02&87\%&70\%&-0.08&90\%&92\%\\
\end{tabular}
\tablefoot{The redshift bins, derived $\alpha_1$ ($\alpha_2$), purity and completeness of `SF' (`QU') samples compared to GAMA catalog.}
\end{center}
\end{table*}

\begin{table}[h]
\begin{center}
\caption{The purity of star-forming and quiescent population compared to red sequence model}
\label{Tab_purity_rs}
\begin{tabular}{cccc} 
\hline
\hline
{$\rm log_{10}(M_*/M_\odot)$} & star-forming&quiescent\\
\hline
(9.5,10.0)&97\%&90\%\\
(10.0,10.5)&90\%&98\%\\
(10.5,11.0)&82\%&96\%\\
(11.0,11.25)&89\%&93\%\\
(11.25,11.5)&78\%&97\%\\
(11.5,12.0)&70\%&99\%\\
\end{tabular}
\tablefoot{The stellar mass bins, the purity of our defined `SF' and `QU' sample compared to the red sequence model derived from galaxy cluster.}
\end{center}
\end{table}

We define the `SF' and `QU' samples of LS DR9 catalog according to the color magnitude diagram.
We use GAMA to constrain the separation of `SF' and `QU' samples in the color magnitude diagram. 
With SED fitting, GAMA catalog provides accurate estimation of SFRs of galaxies. We define GAMA galaxy with specific star formation rate $log(sSFR)> -10.5 yr^{-1}$ as star-forming galaxy and $log(sSFR)< -10.5 yr^{-1}$ as quiescent galaxy \citep{Belfiore2018}.
%This definition gives similar SMF to \citet{Kelvin2014}

We take the matched galaxies in Section.~\ref{Apd_dr9_gama_cat}.
The quality of `SF' and `QU' sample definition is quantified by the purity and completeness. 
The purity is defined as the percentage of LS DR9 galaxies identified as `SF' and `QU' also in GAMA. The completeness is defined as the percentage of `SF' and `QU' in GAMA also in LS DR9.

We fix the slope of the separation and change $\alpha_1$ and $\alpha_2$ to find the values where the purity of `SF' and `QU' samples is about 90\% and not losing the completeness.
The magnitude we used have considered Galactic extinction \citep{Zou2019}. The results at different redshift bins are listed in Table.~\ref{Tab_purity}.
As an example, the color-magnitude diagram of matched galaxies at $z<0.1$ is plotted in Fig.~\ref{Fig_gama_dr9_color}.
We then applied another check by comparing to the red sequence model defined in . We take the definition of red sequence and calculate the purity again, the result is listed in Table.~\ref{Tab_purity_rs}.
%GAMA can be split to blue/green/red galaxies according to the colour– mass diagram \citep{Prescott2011}. The separation between blue and green (green and red) is $(g-i)=0.03\times log(M_*) +0.45 (0.4)$. 
%The two definitions agree with each other, as plotted in Fig.`\ref{Fig_gama_rgb}'
In general, our LS red sequence galaxy is well defined with high purity and completeness.

%\section{Needed $z_{spec}$ to selection central galaxy} \label{Apd_specz}

%We define central galaxy as the most massive galaxy that has no intersect within two times of its virial radius in space. We find even using spectroscopic survey that can estimate redshift with $\Delta z<0.0001$, there are still $>30\&$ satellite galaxies wrongly pass the central galaxy selection. Therefore with the LS DR9 galaxy catalog where $\Delta z \approx 0.01$, it is impossible to separate central and satellite galaxies correctly. 

%Besides, we add the typical error of spectropic redshift ($\Delta z_{spec}=0.0001$ \citep{Driver2022,Strauss2002,Thomas2013}) to Uchuu catalog and do the 3D selection, the HOD is plotted in . 

\section{AGN models for star-forming and quiescent galaxies}\label{Apd_agn}


As shown in the left panel, for the MW-mass galaxies, the predicted AGN emission is brighter than the detection within about 50 kpc. The AGN model overestimates the X-ray emission.
The maximum emission from the AGN and XRB in the stacked galaxies should be in the shape of PSF, with the first bin as bright as detected, as the blue dots show. We integrate the maximum emission and compare it to the predicted AGN and XRB emission at other $M_*$ bins, as plotted in the right panel. The AGN model overestimates the X-ray emission in the galaxy for most cases. After masking X-ray sources, the contamination from bright AGN is reduced, but the predicted AGN is still too bright, as plotted in Fig.~\ref{Fig_agn_cen}. Generally, the predicted AGN is about 0.7-8 times of the detected maximal AGN luminosity.
The failure of the AGN model is due to the low redshift we are looking at. Limited by previous X-ray surveys, the sample of AGN in low redshift is small, though the AGN model works well at higher redshift, the AGN model is poorly constrained in $z<0.5$ and $L_{\rm X,2-10 keV}<10^{41} \rm erg/s$. 

Measuring unbiased stellar masses in the presence of AGN light is notoriously difficult (Ciesla et al. 2015, Buchner et al. in prep). The masses used in this analysis are not inferred using models that includes an AGN (Zou et al. 2019). It means that systematically, stellar masses of galaxies hosting AGN will be over-estimated. 
This in turn forces us to model the AGN contamination from the observer perspective. Indeed using simulation with perfect stellar mass information will then over-estimate possible AGN contamination.

Therefore instead of using the existing AGN model, we estimate the AGN contamination in the `CEN' sample by stacking of galaxies hosting AGN. We select the galaxies hosting AGN, identified as AGN or composite, based on the BPT diagram \citep{BPT1981,Brichmann2004}. We name the AGN sample as `CENAGN'. The percentage of `CEN' galaxies identified as hosting AGN ($f_{\rm AGN}$) is about 8-18\%, as listed in Table.~\ref{Tab_cenagn}. We stack the `CENAGN' sample and calculate the maximum X-ray emission from AGN and XRB as described above. The maximal AGN emission ($L_{\rm AGN,max}$) is the residual emission after subtracting the XRB emission. Under the assumption of no other galaxies hosting AGN, the lower limit of the average AGN contamination in `CEN' sample is therefore $L_{\rm AGN,max}\times f_{\rm AGN}$. To be conservative, we take the upper limit of AGN contamination as $2\times L_{\rm AGN,max}\times f_{\rm AGN}$. 
We can only overestimate the AGN, as the BPT diagram selects the star-forming galaxies, where the AGN incidence is about 10 times higher than quiescent galaxies \citep{Aird2018}. 

The estimated AGN contamination is plotted in . When X-ray sources are masked, the unresolved AGN contamination is less than 30\% of XRB emission. 

\begin{table*}[h]
\begin{center}
\caption{The percentage and number of galaxy hosting AGN in `CEN' sample, identified using the BPT diagram \citep{BPT1981,Brichmann2004}. }
\label{Tab_cenagn}
\begin{tabular}{ccccccccc} 
\hline
\hline
$\log(M_*)$ &$f_{\rm AGN}$ &$N_{\rm CENAGN}$&$f_{\rm AGN,SF}$ &$N_{\rm CENAGN,SF}$&$f_{\rm AGN,QU}$ &$N_{\rm CENAGN,QU}$\\
\hline
10.0-10.5&16\%&1261&13\%&699&22\%&562\\
10.5-11.0&18\%&5421&24\%&3377&12\%&2044\\
11.0-11.25&14\%&3447&28\%&2367&6\%&1080\\
11.25-11.5&8\%&1505&22\%&964&3\%&541\\
\end{tabular}
\end{center}
\end{table*}


In this work, to resolve CGM, we masked detected X-ray sources. Here we stack the `CEN' galaxies hosting AGN (in BPT diagram), therefore the AGN contamination is maximal, and compared to the stack of `CEN' galaxies (both apply mask). We find the two stacks give consistent results, which means the AGN contamination is ignorable when X-ray sources are masked. 

The galaxies hosting AGN are defined based on the BPT diagram \citep{BPT1981,Brichmann2004}. We stack these galaxies.




Therefore, we take the maximum emission constrained by the stack profile to count for the AGN and XRB emission in the stacked galaxies.

Except the AGNs and XRBs in the stacked galaxies contributing to the stacking result, the X-ray emission from the AGN and XRB in the surrounding satellite galaxies is stacked to the result. The model of the X-ray emission of it is plotted in Fig.~\ref{Fig_agn_sat}. For the MW-mass galaxies, the emission of AGN and XRB in the satellite is low but starts to matter beyond 100 kpc. The comparison of the AGN and XRB luminosity is in the right panel. 
The AGN models overestimate the X-ray emission, therefore we take the emission of AGN and XRB in the satellite as an up-limit. The total AGN and XRB emission is the sum of the maximum emission in stacked galaxies and the modeled emission in satellite galaxies.

To make the faint CGM emission more discernible, we mask all detected X-ray sources. To model the masking, we applied a flux cut to the modeled AGN flux as a function to the $t_{\rm exp}$. Here we compare the masked X-ray luminosity to the modeled masked X-ray luminosity to validate the flux limit cut. The comparison is in Fig.~\ref{Fig_agn_mask}. The modeled masked AGN emission is comparable or lower than the masked X-ray emission in the stack. Considering the masked emission is all detected X-ray sources, not all AGN, we think the flux limit is proper.

\section{Results not presented in main text} \label{Apd_profiles}
\subsection{X-ray surface brightness profiles} 

fullphot 9.5-,11.25- nomask profiles, with mask profiles.
with mask, isolated+cen, 11.25-11.5,9.5- profiles.
\subsection{X-ray luminosity within $R_{vir}$}\label{Apd_lxvir}

\subsection{Lx-M relation for sf/qu without mask}
\begin{figure}
    \centering
    \includegraphics[width=1.0\columnwidth]{fig/lxm/lx_m_halo_nomask_cen_sfqu_R500.png}

    \caption{Left: The X-ray luminosity $R_{500}$ as a function of the $M_{halo}$ for dark matter halos ting star-forming or quiescent central galaxies respectively. The dashed line is a linear relation for illustration and does not fit the data.}
        \label{Fig_lxm_halosfqu}
\end{figure}



\section{Compare the X-ray surface brightness profiles of isolated and CEN samples} \label{Apd_isocen}

\begin{figure*}
    \centering
    \includegraphics[width=1.0\columnwidth]{fig/profile/profile_nomask_2dcen_M31_gal.png}
    \includegraphics[width=1.0\columnwidth]{fig/profile/profile_mask_2dcen_M31_gal.png}
    \caption{The X-ray surface brightness profiles (points) of M31-mass galaxies from isolated and CEN samples after subtracting background, without (left) and with (right) masking X-ray sources. The dotted line is the PSF of eROSITA.}
        \label{Fig_profile_2dcen}
\end{figure*}

The comparison of the X-ray surface brightness profiles of isolated and CEN samples, taking the M31-mass bin as an example, is shown in Fig.~\ref{Fig_profile_2dcen}. 
When the bright point sources in the stacked galaxies are not masked, the observed X-ray surface brightness profile of the isolated galaxies is close to the PSF shape. The X-ray surface brightness profile of the CEN sample is sharper than isolated galaxies within 100 kpc. This is due to the lower average redshift of the CEN sample (limited by the magnitude limit of SDSS, $r_{\rm AB}<17.77$), that the PSF in the physical scale is smaller. 
Beyond about 100 kpc, where the PSF influence is low, the X-ray emission of CEN and isolated galaxies is comparable. 

Due to the selection criteria of the isolated sample, we expect it to have lower X-ray emission from the satellite galaxies than the CEN sample, which would sharpen the X-ray profile of the isolated sample.
However, we did not detect this feature, limited by the statistics. 

The other influence of the different redshift distributions of isolated and CEN samples is the masking of X-ray sources. Because the isolated sample has a higher average redshift, fewer X-ray sources are detected. The X-ray surface brightness profile of the isolated sample after masking X-ray sources is slightly higher than the CEN sample (see the right panel of Fig.~\ref{Fig_profile_2dcen}).

\section{Model the misclassified central galaxies}\label{Sec_profilesat}

\begin{figure*}
    \centering
    \includegraphics[width=1.0\columnwidth]{fig/profile/profile_nomask_censat_M31_gal.png}
        \includegraphics[width=1.0\columnwidth]{fig/profile/profile_nomask_censat_M31_gal_norm.png}
    \caption{Left: The average X-ray surface brightness profile of galaxies in M31-mass bin and profiles after splitting to central (CEN) or satellite (SAT) galaxies. Right: Surface brightness profiles of galaxies in M31-mass bin after rescaling $S_X$ of central and satellite samples according to the galaxy number. }
        \label{Fig_profile_censat}
\end{figure*}

We learned the satellite boost biases the stacking, in this section, we stack the X-ray emission around satellite galaxies to build a model of satellite boost, which can untangle the X-ray surface brightness profile of central galaxies from the stacking of FULL$_{\rm phot}$ sample. 

The X-ray surface brightness profiles of 

The comparison of X-ray surface brightness profile of satellite galaxy to central galaxy and all galaxies is plotted in Fig.~\ref{Fig_profile_censat}, take the M31-mass bin as an example. 
The galaxies with same $M_*$ but being satellite or central have different X-ray surface brightness profiles. The satellite galaxy, residing in more massive dark matter halo, its X-ray emission is boosted by emission from virialized gas, nearby central and other satellite galaxies. The X-ray surface brightness profile of satellite galaxy appears to be more extended and brighter than central galaxy.  

We then interpret the surface brightness profile of FULL$_{\rm phot}$ sample. We rescale the profile of central or satellite galaxy by their number ratio, namely times the profile by $N_{CEN}/N_g$ or $N_{SAT}/N_g$. The rescaled profiles of central and satellite comparing to the FULL$_{\rm phot}$ sample is plotted in the right panel of Fig.~\ref{Fig_profile_censat}. Beyond 100 kpc, the emission from satellite galaxies dominates over central galaxy and decides the profile shape of FULL$_{\rm phot}$ sample. This proves the necessity of selecting isolated or central galaxies to study how galaxy modulates the properties of its CGM. On the other hand, we can use the rescaled profiles to untangle the emission in FULL$_{\rm phot}$ sample, the detail is discussed in Sec.~\ref{}

We model it using four parameters with 
\begin{equation}
\label{Eq:satFrac}
\left(\frac{1}{2} + \frac{1}{2} erf\left(\frac{\log_{10}(R_p)-\log_{10}(R_0)}{\sigma}\right)\right)\times (y_1-y_0) + y_0
\end{equation}
The best-fit parameters (with a simple $\chi^2$ minimization routine) are given in Table


\jc{this likely goes to fast, you need to explain that the you have the CEN and SAT intrinsic SB profiles tabulated for a given selection in stellar mass. Then you can fit the measured FULL sample stack with adjusting the f sat parameter to (1-fsat)xCEN + (fsat)xSAT. Then compare the fsat you obtain to that predicted by Uchuu mock catalogues. If in agreement, you can claim that you can correct the FULL sample from satellite contamination. Finally you show the central component of the FULL stack and compare it to the isolated and CEN stack. Hopefully, they agree but the FULL central component has a higher signal to noise ratio. Maybe then you can claim an even higher significance of detection of extended emission for MW-mass or M31-mass.}



\section{Compare to \citet{Comparat2022} and \citet{Chada2022}} \label{Apd_comparesfqu}

\begin{figure*}
    \centering
    \includegraphics[width=0.33\linewidth]{fig/discuss/lx_m_compare_johan.png}
    \includegraphics[width=0.33\linewidth]{fig/discuss/lx_m_compare_chada.png}
    \caption{\jc{for the comparisons, are you using similarly designed samples ? The isolated samples should not be directly compared to the eFEDS results. Rather the full sample (that includes satellite contamination) should.}}
        \label{Fig_compare}
\end{figure*}

Use the released eFEDS data, which covers a sky area of $140 \rm deg^2$, there were two papers studying the hot gas around star-forming and quiescent galaxies by stacking. 
\citet{Comparat2022} stacked 16142 galaxies at 0.05$\le z_{spec} \le$ 0.3 taken from the GAMA spectroscopic survey. They found the X-ray profile and luminosity trends in quiescent and star-forming galaxy populations are different at lower mass, that quiescent galaxies are brighter and more extended, without masking of detected galaxy groups or galaxy clusters. 
\citet{Chada2022} stacked 1643 galaxies at 0.01<$z_{spec}$<0.1 selected from \citep{Ahn2014,Montero2016}. They masked all X-ray sources out and found that star-forming galaxies are brighter than quiescent galaxies.
We compare the X-ray data and galaxy samples used in these two papers and our work in Table~\ref{Tab_compare}. 


%Except for the redshift bin, the main difference between the galaxy samples in the two works is that \citet{Comparat2022} selected central galaxies \footnote{defined as the most massive galaxy within, though the selection is not good enough as we discussed in the Appendix.~\ref{}.} and \citet{Chada2022} do not apply selection. 

and this work selected 'isolated' galaxies. We apply the two different galaxy selections to Uchuu galaxy catalog. We compare the selected galaxy in $10.7<log(M_*)<11.2$ bin, namely the MW to M31 like galaxies.
In Fig.~\ref{Fig_hod_compare}, the number of central and satellite galaxies kept in the sample as a function of mass of dark matter halo is plotted. 
The central galaxies at $10.7<log(M_*)<11.2$ are mainly tracing $1-3\times10^{12}M_\odot$ dark matter halo, while the satellite galaxies locate in more massive dark matter halo.
The galaxy samples of \citet{Chada2022} and \citet{Comparat2022} are similarly distributed in dark matter halo, \citet{Chada2022} kept all satellite galaxies and \citet{Comparat2022} removed about 10\% satellite galaxies. Our 'isolated' sample removed most satellist galaxies.

%The background in \citet{Chada2022} is calculated from the ring 150-300 kpc, \citet{Comparat2022} took the average background in efeds area. We take the background where the X-ray emission profile decreases to stable flux. 

\begin{table*}[h]
\begin{center}
\caption{Comparison to previous stacking works.}
\label{Tab_compare}
\begin{tabular}{cccccccccc} 
\hline
\hline
&\citeauthor{Anderson2015} &\citeauthor{Comparat2022} & \citeauthor{Chada2022} &\multicolumn{2}{c}{This work}\\
&(\citeyear{Anderson2015})&(\citeyear{Comparat2022})&(\citeyear{Chada2022})&Isolated&`CEN'\\
\hline
X-ray data&ROSAT & eFEDS & eFEDS & eRASS:4& eRASS:4\\ 
$t_{\rm exp,med}$&0.3ks&1.2ks&1.2ks&0.55ks&0.55ks\\
stack area ($\rm deg^2$)&6800 &60&140&9340&4010\\
\hline
Galaxy catalog&SDSS &GAMA&SDSS MGS&DESI LS DR9 &SDSS MGS\\
Redshift&0.04$\le z_{\rm spec}\le$0.4&0.05$\le z_{\rm spec} \le$ 0.3& 0.01$\le z_{\rm spec}\le$0.1&0.01$\le z_{\rm phot} \le$0.4&0.01$\le z_{\rm spec} \le$0.19\\ 
$\log(M_*)$ bin&10.0-12.0& 9.5-12.0& 10.2-11.2& 9.5-11.5 & 10.0-11.5 \\
Galaxy selection&central galaxy&central galaxy & - & isolated galaxy&central galaxy \\
Galaxy number&259567 &16142 &1643 &213514&85222 \\
SF/QU definition&- &sSFR&sSFR&color-magnitude&4000\AA \ break\\
%Background &random area near galaxy&150-300kpc&random area near galaxy\\
\end{tabular}
\tablefoot{We list the difference of used X-ray data and galaxy sample in \citet{Comparat2022}, \citet{Chada2022} and our work.}
\end{center}
\end{table*}







%On the other hand, the discrepancy above caused by trivial galaxy sample definition implies why different conclusions were drawn from different stackings. The accurate selection and sufficient understanding of galaxy samples are important to do stacking analysis without bias. 

\end{appendix}





\end{document}

\section{star-forming and quiescent population definition of LS DR9}
\label{Apd_sfqu}

\begin{figure}
     \centering
         \includegraphics[width=0.8\columnwidth]{fig/apd/DR9_GAMA_color.png}
        \caption{The color-magnitude diagram of the LS DR9 sample matched to GAMA at $z<0.1$. The color of the dots denote the star-forming or quiescent defined in GAMA. The line separate the star-forming (below line) or quiescent (above line) galaxies in LS DR9.}
        \label{Fig_gama_dr9_color}
\end{figure}

\begin{table*}[h]
\begin{center}
\caption{The completeness and purity of star-forming and quiescent population definition}
\label{Tab_purity}
\begin{tabular}{c|ccc|cccc} 
\hline
\hline
&&star-forming&&&quiescent&\\

&$\alpha_1$&purity&completeness&$\alpha_2$&purity&completeness\\
\hline
z<0.1&0.37&90\%&91\%&0.34&88\%&78\%\\
0.1<z<0.2&0.33&89\%&76\%&0.29&89\%&90\%\\
0.2<z<0.3&0.12&88\%&79\%&0.06&88\%&85\%\\
0.3<z<0.4&-0.02&87\%&70\%&-0.08&90\%&92\%\\
\end{tabular}
\tablefoot{The redshift bins, derived $\alpha_1$ ($\alpha_2$), purity and completeness of `SF' (`QU') samples compared to GAMA catalog.}
\end{center}
\end{table*}

\begin{table}[h]
\begin{center}
\caption{The purity of star-forming and quiescent population compared to red sequence model}
\label{Tab_purity_rs}
\begin{tabular}{cccc} 
\hline
\hline
{$\rm log_{10}(M_*/M_\odot)$} & star-forming&quiescent\\
\hline
(9.5,10.0)&97\%&90\%\\
(10.0,10.5)&90\%&98\%\\
(10.5,11.0)&82\%&96\%\\
(11.0,11.25)&89\%&93\%\\
(11.25,11.5)&78\%&97\%\\
(11.5,12.0)&70\%&99\%\\
\end{tabular}
\tablefoot{The stellar mass bins, the purity of our defined `SF' and `QU' sample compared to the red sequence model derived from galaxy cluster.}
\end{center}
\end{table}

We define the `SF' and `QU' samples of LS DR9 catalog according to the color magnitude diagram.
We use GAMA to constrain the separation of `SF' and `QU' samples in the color magnitude diagram. 
With SED fitting, GAMA catalog provides accurate estimation of SFRs of galaxies. We define GAMA galaxy with specific star formation rate $log(sSFR)> -10.5 yr^{-1}$ as star-forming galaxy and $log(sSFR)< -10.5 yr^{-1}$ as quiescent galaxy \citep{Belfiore2018}.
%This definition gives similar SMF to \citet{Kelvin2014}

We take the matched galaxies in Section.~\ref{Apd_dr9_gama_cat}.
The quality of `SF' and `QU' sample definition is quantified by the purity and completeness. 
The purity is defined as the percentage of LS DR9 galaxies identified as `SF' and `QU' also in GAMA. The completeness is defined as the percentage of `SF' and `QU' in GAMA also in LS DR9.

We fix the slope of the separation and change $\alpha_1$ and $\alpha_2$ to find the values where the purity of `SF' and `QU' samples is about 90\% and not losing the completeness.
The magnitude we used have considered Galactic extinction \citep{Zou2019}. The results at different redshift bins are listed in Table.~\ref{Tab_purity}.
As an example, the color-magnitude diagram of matched galaxies at $z<0.1$ is plotted in Fig.~\ref{Fig_gama_dr9_color}.
We then applied another check by comparing to the red sequence model defined in . We take the definition of red sequence and calculate the purity again, the result is listed in Table.~\ref{Tab_purity_rs}.
%GAMA can be split to blue/green/red galaxies according to the colour– mass diagram \citep{Prescott2011}. The separation between blue and green (green and red) is $(g-i)=0.03\times log(M_*) +0.45 (0.4)$. 
%The two definitions agree with each other, as plotted in Fig.`\ref{Fig_gama_rgb}'
In general, our LS red sequence galaxy is well defined with high purity and completeness.

%\section{Needed $z_{spec}$ to selection central galaxy} \label{Apd_specz}

%We define central galaxy as the most massive galaxy that has no intersect within two times of its virial radius in space. We find even using spectroscopic survey that can estimate redshift with $\Delta z<0.0001$, there are still $>30\&$ satellite galaxies wrongly pass the central galaxy selection. Therefore with the LS DR9 galaxy catalog where $\Delta z \approx 0.01$, it is impossible to separate central and satellite galaxies correctly. 

%Besides, we add the typical error of spectropic redshift ($\Delta z_{spec}=0.0001$ \citep{Driver2022,Strauss2002,Thomas2013}) to Uchuu catalog and do the 3D selection, the HOD is plotted in . 

\section{Results not presented in main text} \label{Apd_profiles}
\subsection{X-ray surface brightness profiles} 

fullphot 9.5-,11.25- nomask profiles, with mask profiles.
with mask, isolated+cen, 11.25-11.5,9.5- profiles.
\subsection{X-ray luminosity within $R_{vir}$}\label{Apd_lxvir}

\subsection{Lx-M relation for sf/qu without mask}
\begin{figure}
    \centering
    \includegraphics[width=1.0\columnwidth]{fig/lxm/lx_m_halo_nomask_cen_sfqu_R500.png}

    \caption{Left: The X-ray luminosity $R_{500}$ as a function of the $M_{halo}$ for dark matter halos ting star-forming or quiescent central galaxies respectively. The dashed line is a linear relation for illustration and does not fit the data.}
        \label{Fig_lxm_halosfqu}
\end{figure}



\section{Compare the X-ray surface brightness profiles of isolated and CEN samples} \label{Apd_isocen}

\begin{figure*}
    \centering
    \includegraphics[width=1.0\columnwidth]{fig/profile/profile_nomask_2dcen_M31_gal.png}
    \includegraphics[width=1.0\columnwidth]{fig/profile/profile_mask_2dcen_M31_gal.png}
    \caption{The X-ray surface brightness profiles (points) of M31-mass galaxies from isolated and CEN samples after subtracting background, without (left) and with (right) masking X-ray sources. The dotted line is the PSF of eROSITA.}
        \label{Fig_profile_2dcen}
\end{figure*}

The comparison of the X-ray surface brightness profiles of isolated and CEN samples, taking the M31-mass bin as an example, is shown in Fig.~\ref{Fig_profile_2dcen}. 
When the bright point sources in the stacked galaxies are not masked, the observed X-ray surface brightness profile of the isolated galaxies is close to the PSF shape. The X-ray surface brightness profile of the CEN sample is sharper than isolated galaxies within 100 kpc. This is due to the lower average redshift of the CEN sample (limited by the magnitude limit of SDSS, $r_{\rm AB}<17.77$), that the PSF in the physical scale is smaller. 
Beyond about 100 kpc, where the PSF influence is low, the X-ray emission of CEN and isolated galaxies is comparable. 

Due to the selection criteria of the isolated sample, we expect it to have lower X-ray emission from the satellite galaxies than the CEN sample, which would sharpen the X-ray profile of the isolated sample.
However, we did not detect this feature, limited by the statistics. 

The other influence of the different redshift distributions of isolated and CEN samples is the masking of X-ray sources. Because the isolated sample has a higher average redshift, fewer X-ray sources are detected. The X-ray surface brightness profile of the isolated sample after masking X-ray sources is slightly higher than the CEN sample (see the right panel of Fig.~\ref{Fig_profile_2dcen}).

\section{Model the misclassified central galaxies}\label{Sec_profilesat}

\begin{figure*}
    \centering
    \includegraphics[width=1.0\columnwidth]{fig/profile/profile_nomask_censat_M31_gal.png}
        \includegraphics[width=1.0\columnwidth]{fig/profile/profile_nomask_censat_M31_gal_norm.png}
    \caption{Left: The average X-ray surface brightness profile of galaxies in M31-mass bin and profiles after splitting to central (CEN) or satellite (SAT) galaxies. Right: Surface brightness profiles of galaxies in M31-mass bin after rescaling $S_X$ of central and satellite samples according to the galaxy number. }
        \label{Fig_profile_censat}
\end{figure*}

We learned the satellite boost biases the stacking, in this section, we stack the X-ray emission around satellite galaxies to build a model of satellite boost, which can untangle the X-ray surface brightness profile of central galaxies from the stacking of FULL$_{\rm phot}$ sample. 

The X-ray surface brightness profiles of 

The comparison of X-ray surface brightness profile of satellite galaxy to central galaxy and all galaxies is plotted in Fig.~\ref{Fig_profile_censat}, take the M31-mass bin as an example. 
The galaxies with same $M_*$ but being satellite or central have different X-ray surface brightness profiles. The satellite galaxy, residing in more massive dark matter halo, its X-ray emission is boosted by emission from virialized gas, nearby central and other satellite galaxies. The X-ray surface brightness profile of satellite galaxy appears to be more extended and brighter than central galaxy.  

We then interpret the surface brightness profile of FULL$_{\rm phot}$ sample. We rescale the profile of central or satellite galaxy by their number ratio, namely times the profile by $N_{CEN}/N_g$ or $N_{SAT}/N_g$. The rescaled profiles of central and satellite comparing to the FULL$_{\rm phot}$ sample is plotted in the right panel of Fig.~\ref{Fig_profile_censat}. Beyond 100 kpc, the emission from satellite galaxies dominates over central galaxy and decides the profile shape of FULL$_{\rm phot}$ sample. This proves the necessity of selecting isolated or central galaxies to study how galaxy modulates the properties of its CGM. On the other hand, we can use the rescaled profiles to untangle the emission in FULL$_{\rm phot}$ sample, the detail is discussed in Sec.~\ref{}

We model it using four parameters with 
\begin{equation}
\label{Eq:satFrac}
\left(\frac{1}{2} + \frac{1}{2} erf\left(\frac{\log_{10}(R_p)-\log_{10}(R_0)}{\sigma}\right)\right)\times (y_1-y_0) + y_0
\end{equation}
The best-fit parameters (with a simple $\chi^2$ minimization routine) are given in Table


\jc{this likely goes to fast, you need to explain that the you have the CEN and SAT intrinsic SB profiles tabulated for a given selection in stellar mass. Then you can fit the measured FULL sample stack with adjusting the f sat parameter to (1-fsat)xCEN + (fsat)xSAT. Then compare the fsat you obtain to that predicted by Uchuu mock catalogues. If in agreement, you can claim that you can correct the FULL sample from satellite contamination. Finally you show the central component of the FULL stack and compare it to the isolated and CEN stack. Hopefully, they agree but the FULL central component has a higher signal to noise ratio. Maybe then you can claim an even higher significance of detection of extended emission for MW-mass or M31-mass.}








%On the other hand, the discrepancy above caused by trivial galaxy sample definition implies why different conclusions were drawn from different stackings. The accurate selection and sufficient understanding of galaxy samples are important to do stacking analysis without bias. 

\section{AGN models for star-forming and quiescent galaxies}\label{Apd_agn}


As shown in the left panel, for the MW-mass galaxies, the predicted AGN emission is brighter than the detection within about 50 kpc. The AGN model overestimates the X-ray emission.
The maximum emission from the AGN and XRB in the stacked galaxies should be in the shape of PSF, with the first bin as bright as detected, as the blue dots show. We integrate the maximum emission and compare it to the predicted AGN and XRB emission at other $M_*$ bins, as plotted in the right panel. The AGN model overestimates the X-ray emission in the galaxy for most cases. After masking X-ray sources, the contamination from bright AGN is reduced, but the predicted AGN is still too bright, as plotted in Fig.~\ref{Fig_agn_cen}. Generally, the predicted AGN is about 0.7-8 times of the detected maximal AGN luminosity.
The failure of the AGN model is due to the low redshift we are looking at. Limited by previous X-ray surveys, the sample of AGN in low redshift is small, though the AGN model works well at higher redshift, the AGN model is poorly constrained in $z<0.5$ and $L_{\rm X,2-10 keV}<10^{41} \rm erg/s$. 

Measuring unbiased stellar masses in the presence of AGN light is notoriously difficult (Ciesla et al. 2015, Buchner et al. in prep). The masses used in this analysis are not inferred using models that includes an AGN (Zou et al. 2019). It means that systematically, stellar masses of galaxies hosting AGN will be over-estimated. 
This in turn forces us to model the AGN contamination from the observer perspective. Indeed using simulation with perfect stellar mass information will then over-estimate possible AGN contamination.

Therefore instead of using the existing AGN model, we estimate the AGN contamination in the `CEN' sample by stacking of galaxies hosting AGN. We select the galaxies hosting AGN, identified as AGN or composite, based on the BPT diagram \citep{BPT1981,Brichmann2004}. We name the AGN sample as `CENAGN'. The percentage of `CEN' galaxies identified as hosting AGN ($f_{\rm AGN}$) is about 8-18\%, as listed in Table.~\ref{Tab_cenagn}. We stack the `CENAGN' sample and calculate the maximum X-ray emission from AGN and XRB as described above. The maximal AGN emission ($L_{\rm AGN,max}$) is the residual emission after subtracting the XRB emission. Under the assumption of no other galaxies hosting AGN, the lower limit of the average AGN contamination in `CEN' sample is therefore $L_{\rm AGN,max}\times f_{\rm AGN}$. To be conservative, we take the upper limit of AGN contamination as $2\times L_{\rm AGN,max}\times f_{\rm AGN}$. 
We can only overestimate the AGN, as the BPT diagram selects the star-forming galaxies, where the AGN incidence is about 10 times higher than quiescent galaxies \citep{Aird2018}. 

The estimated AGN contamination is plotted in . When X-ray sources are masked, the unresolved AGN contamination is less than 30\% of XRB emission. 

\begin{table*}[h]
\begin{center}
\caption{The percentage and number of galaxy hosting AGN in `CEN' sample, identified using the BPT diagram \citep{BPT1981,Brichmann2004}. }
\label{Tab_cenagn}
\begin{tabular}{ccccccccc} 
\hline
\hline
$\log(M_*)$ &$f_{\rm AGN}$ &$N_{\rm CENAGN}$&$f_{\rm AGN,SF}$ &$N_{\rm CENAGN,SF}$&$f_{\rm AGN,QU}$ &$N_{\rm CENAGN,QU}$\\
\hline
10.0-10.5&16\%&1261&13\%&699&22\%&562\\
10.5-11.0&18\%&5421&24\%&3377&12\%&2044\\
11.0-11.25&14\%&3447&28\%&2367&6\%&1080\\
11.25-11.5&8\%&1505&22\%&964&3\%&541\\
\end{tabular}
\end{center}
\end{table*}


In this work, to resolve CGM, we masked detected X-ray sources. Here we stack the `CEN' galaxies hosting AGN (in BPT diagram), therefore the AGN contamination is maximal, and compared to the stack of `CEN' galaxies (both apply mask). We find the two stacks give consistent results, which means the AGN contamination is ignorable when X-ray sources are masked. 

The galaxies hosting AGN are defined based on the BPT diagram \citep{BPT1981,Brichmann2004}. We stack these galaxies.




Therefore, we take the maximum emission constrained by the stack profile to count for the AGN and XRB emission in the stacked galaxies.

Except the AGNs and XRBs in the stacked galaxies contributing to the stacking result, the X-ray emission from the AGN and XRB in the surrounding satellite galaxies is stacked to the result. The model of the X-ray emission of it is plotted in Fig.~\ref{Fig_agn_sat}. For the MW-mass galaxies, the emission of AGN and XRB in the satellite is low but starts to matter beyond 100 kpc. The comparison of the AGN and XRB luminosity is in the right panel. 
The AGN models overestimate the X-ray emission, therefore we take the emission of AGN and XRB in the satellite as an up-limit. The total AGN and XRB emission is the sum of the maximum emission in stacked galaxies and the modeled emission in satellite galaxies.

To make the faint CGM emission more discernible, we mask all detected X-ray sources. To model the masking, we applied a flux cut to the modeled AGN flux as a function to the $t_{\rm exp}$. Here we compare the masked X-ray luminosity to the modeled masked X-ray luminosity to validate the flux limit cut. The comparison is in Fig.~\ref{Fig_agn_mask}. The modeled masked AGN emission is comparable or lower than the masked X-ray emission in the stack. Considering the masked emission is all detected X-ray sources, not all AGN, we think the flux limit is proper.




%The background in \citet{Chada2022} is calculated from the ring 150-300 kpc, \citet{Comparat2022} took the average background in efeds area. We take the background where the X-ray emission profile decreases to stable flux. 

\begin{table*}[h]
\begin{center}
\caption{Comparison to previous stacking works.}
\label{Tab_compare}
\begin{tabular}{cccccccccc} 
\hline
\hline
&\citeauthor{Anderson2015} &\citeauthor{Comparat2022} & \citeauthor{Chada2022} &\multicolumn{2}{c}{This work}\\
&(\citeyear{Anderson2015})&(\citeyear{Comparat2022})&(\citeyear{Chada2022})&Isolated&`CEN'\\
\hline
X-ray data&ROSAT & eFEDS & eFEDS & eRASS:4& eRASS:4\\ 
$t_{\rm exp,med}$&0.3ks&1.2ks&1.2ks&0.55ks&0.55ks\\
stack area ($\rm deg^2$)&6800 &60&140&9340&4010\\
\hline
Galaxy catalog&SDSS &GAMA&SDSS MGS&DESI LS DR9 &SDSS MGS\\
Redshift&0.04$\le z_{\rm spec}\le$0.4&0.05$\le z_{\rm spec} \le$ 0.3& 0.01$\le z_{\rm spec}\le$0.1&0.01$\le z_{\rm phot} \le$0.4&0.01$\le z_{\rm spec} \le$0.19\\ 
$\log(M_*)$ bin&10.0-12.0& 9.5-12.0& 10.2-11.2& 9.5-11.5 & 10.0-11.5 \\
Galaxy selection&central galaxy&central galaxy & - & isolated galaxy&central galaxy \\
Galaxy number&259567 &16142 &1643 &213514&85222 \\
SF/QU definition&- &sSFR&sSFR&color-magnitude&4000\AA \ break\\
%Background &random area near galaxy&150-300kpc&random area near galaxy\\
\end{tabular}
\tablefoot{We list the difference of used X-ray data and galaxy sample in \citet{Comparat2022}, \citet{Chada2022} and our work.}
\end{center}
\end{table*}

